An overview of diffusion models for generative artificial intelligence

This article provides a mathematically rigorous introduction to denoising diffusion probabilistic models (DDPMs), sometimes also referred to as diffusion probabilistic models or diffusion models, for generative artificial intelligence. We provide a detailed basic mathematical framework for DDPMs and explain the main ideas behind training and generation procedures. In this overview article we also review selected extensions and improvements of the basic framework from the literature such as improved DDPMs, denoising diffusion implicit models, classifier-free diffusion guidance models, and latent diffusion models.

==> scheme.tex <==
\def\ConvColor{rgb:yellow,5;red,2.5;white,5}
\def\ConvReluColor{rgb:yellow,5;red,5;white,5}
\def\PoolColor{rgb:red,1;black,0.3}
\def\UnpoolColor{rgb:blue,2;green,1;black,0.3}
\def\ConcatColor{rgb:blue,5;red,2.5;white,5}
\def\FcReluColor{rgb:blue,5;red,5;white,4}
\def\SoftmaxColor{rgb:magenta,5;black,7}


\newcommand{\copymidarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw={rgb:blue,4;red,1;green,1;black,3}] (-0.3,0) -- ++(0.3,0);}

\begin{tikzpicture}
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down},draw=\edgecolor,opacity=0.7]
\tikzstyle{copyconnection}=[ultra thick,every node/.style={sloped,allow upside down},draw={rgb:blue,4;red,1;green,1;black,3},opacity=0.7]

\pic[shift={(0,0,0)}] at (0,0,0) {Box={name=p0,%
     xlabel={{"1\ "," "}},caption= I,fill=\ConvColor,opacity=0.6,height=40,width=1,depth=40}};
\pic[shift={(2,0,0)}] at (p0-west) {RightBandedBox={name=cr1,%
        xlabel={{"64","64"}},caption=I,fill=\ConvColor,bandfill=\ConvReluColor,%
        height=40,width={2,2},depth=40}};
\pic[shift={(1.2,-10,0)}] at (cr1-east) {Box={name=p1,%
     xlabel={{"64"," "}},caption= ,fill=\PoolColor,opacity=0.6,height=32,width=2,depth=32}};

\pic[shift={(0,0,0)}] at (p1-east) {RightBandedBox={name=cr2,%
        xlabel={{"128","128"}},caption =I/2 \ \ \ , fill=\ConvColor,bandfill=\ConvReluColor,%
        height=32,width={4,4},depth=32} };
\pic[shift={(1.2,-8.5,0)}] at (cr2-east) {Box={name=p2,%
        xlabel={{"128"," "}},caption= ,fill=\PoolColor,opacity=0.6,height=16,width=4 ,depth=16}};
\pic[shift={(0,0,0)}] at (p2-east) {RightBandedBox={name=cr3,%
        xlabel={{"256","256"}},caption=I/4\ \ \ \ \ \ \ ,fill=\ConvColor,bandfill=\ConvReluColor,%
        height=16,width={8,8},depth=16}};
\pic[shift={(1.2,-6.5,0)}] at (cr3-east) {Box={name=p3,%
        xlabel={{"256",""}},caption= ,fill=\PoolColor,opacity=0.6,height=8,width=8,depth=8}};

\pic[shift={(0,0,0)}] at (p3-east) {RightBandedBox={name=cr4,caption=I/8 \ \ \ \ \ \ \ \ \ \ \ ,%
        xlabel={{"512","512"}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=8,width={16,16},depth=8}};
\pic[shift={(0,0,0)}] at (cr4-east) {Box={name=ucr3,%
        xlabel={{"256", " "}},caption=I/4,fill=\UnpoolColor,opacity=0.6,height=16,width=8,depth=16}};
\pic[shift={(0,6.5,0)}] at (ucr3-anchor) {Ball={name=cat3,caption= ,fill=\ConcatColor,radius=2.5,logo=$||$}};    
\pic[shift={(1.5,0,0)}] at (cat3-east) {RightBandedBox={name=ucr3a,%
        xlabel={{"256","256"}},caption=I/4,fill=\ConvColor,bandfill=\ConvReluColor,%
        height=16,width={8,8},depth=16}};
\pic[shift={(0,0,0)}] at (ucr3a-east) {Box={name=ucr2,%
        xlabel={{"128","128"}},caption=I/2,fill=\UnpoolColor,opacity=0.6,height=32,width=4,depth=32}};
\pic[shift={(0,8.5,0)}] at (ucr2-anchor) {Ball={name=cat2,caption=I,fill=\ConcatColor,radius=2.5,logo=$||$}};
\pic[shift={(3,0,0)}] at (cat2-east) {RightBandedBox={name=ucr2a,%
        xlabel={{"128","128"}},caption=I/2,fill=\ConvColor,bandfill=\ConvReluColor,%
        height=32,width={4,4},depth=32}};
\pic[shift={(0,0,0)}] at (ucr2a-east) {Box={name=ucr1,%
        xlabel={{"64","64"}},caption=I,fill=\UnpoolColor,opacity=0.6,height=40,width=1,depth=40}};
\pic[shift={(0,10,0)}] at (ucr1-anchor) {Ball={name=cat1,caption=I,fill=\ConcatColor,radius=2.5,logo=$||$}};
\pic[shift={(3.2,0,0)}] at (cat1-east) {RightBandedBox={name=ucr1a,%
        xlabel={{"64","64"}},caption=I,fill=\ConvColor,bandfill=\ConvReluColor,%
        height=40,width={2.5,2.5},depth=40}};
\pic[shift={(2,0,0)}] at (ucr1a-east) {Box={name=out,xlabel={{"1\ "," "}},caption= I,fill=\ConvColor,opacity=0.6,height=40,width=1,depth=40}};
\path (cr1-west) -- (p1-west|-cr1-west) coordinate[pos=0.5] (crp1-mid) ;
\path (cr1-east) -- (p1-west|-cr1-west) coordinate[pos=0.5] (crp1-mid) ;
\path (cr2-east) -- (p2-west|-cr2-west) coordinate[pos=0.5] (crp2-mid) ;
\path (cr3-east) -- (p3-west|-cr3-west) coordinate[pos=0.5] (crp3-mid) ;

\draw[connection](cr1-east)--node{\midarrow}(crp1-mid)--node{\midarrow}(p1-west-|crp1-mid)--node{\midarrow}(p1-west);
\draw[connection](cr2-east)--node{\midarrow}(crp2-mid)--node{\midarrow}(p2-west-|crp2-mid)--node{\midarrow}(p2-west);
\draw[connection](cr3-east)--node{\midarrow}(crp3-mid)--node{\midarrow}(p3-west-|crp3-mid)--node{\midarrow}(p3-west);

\draw [connection]  (ucr1a-east) -- node {\midarrow} (out-west);
\draw [connection]  (p0-east) -- node {\midarrow} (cr1-west);

\draw [copyconnection]  (cr3-east)  -- node {\copymidarrow} (cat3-west);
\draw [copyconnection]  (cr2-east)  -- node {\copymidarrow} (cat2-west);
\draw [copyconnection]  (cr1-east)  -- node {\copymidarrow} (cat1-west);

\draw [copyconnection]  (cat3-east)  -- node {\copymidarrow} (ucr3a-west);
\draw [copyconnection]  (cat2-east)  -- node {\copymidarrow} (ucr2a-west);
\draw [copyconnection]  (cat1-east)  -- node {\copymidarrow} (ucr1a-west);

\draw [copyconnection]  (ucr3-north)  -- node {\copymidarrow} (cat3-south);
\draw [copyconnection]  (ucr2-north)  -- node {\copymidarrow} (cat2-south);
\draw [copyconnection]  (ucr1-north)  -- node {\copymidarrow} (cat1-south);

\end{tikzpicture}

